An MINLP Model for designing decentralized energy supply network

In this report, a detailed description of an MINLP model for decentralized energy supply network optimization is given. This model includes the possibility of extending gas transmission lines, local choice of heating technology, as well as local decisions for energy-efficient house renovation. Ultimately, the model is aimed at finding cost-efficient network plans while reducing carbon emissions to a specified amount.

==> graphics/MECTs.tex <==
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
	%uncomment if require: \path (0,475); %set diagram left start at 0, and has height of 475
	
	%Straight Lines [id:da19227083615185803] 
	\draw [thick, dash pattern={on 5pt off 3pt}]   (71,97.5) -- (71,78.5) -- (293,78.5) ;%(293,77.51) ;
	\draw [shift={(295,78.5)}, rotate = 539.75] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
	%Straight Lines [id:da655808117195579] 
	\draw [thick, dash pattern={on 5pt off 3pt}]   (71,125.5) -- (71,147.5) -- (287,147.5) ;
	\draw [shift={(289,147.5)}, rotate = 180.26] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
	%Straight Lines [id:da23027153476734974] 
	\draw    (111.67,232) -- (449,232) ;
	\draw [shift={(451,232)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
	%Straight Lines [id:da9465914698637938] 
	\draw    (71,219.33) -- (71,190) -- (292.33,190) ;
	\draw [shift={(294.33,190)}, rotate = 180.17] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
	%Straight Lines [id:da891302962287494] 
	\draw    (329,155.33) -- (363,155.33) -- (363,202) -- (480,201.33) -- (480,215.33) ;
	\draw [shift={(480,217.33)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
	%Straight Lines [id:da1786595715386049] 
	\draw [thick, dash dot]  (325.67,192) -- (480,192) -- (480,129.33) ;
	\draw [shift={(480,127.33)}, rotate = 450.6] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
	%Straight Lines [id:da7662454954498437] 
	\draw [thick, dash dot]   (329.67,146) -- (363,146) -- (363,112) -- (461,112) ;
	\draw [shift={(463,112)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
	%Straight Lines [id:da904787856593254] 
	\draw [thick, dash dot]   (323.67,77.33) -- (480,77.33) -- (480,95.33) ;
	\draw [shift={(480,97.33)}, rotate = 268.09000000000003] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
	
	% Text Node
	\draw    (32,99) -- (120,99) -- (120,124) -- (32,124) -- cycle  ;
	\draw (35,103) node [anchor=north west][inner sep=0.75pt]   [align=center] {Natural Gas};
	% Text Node
	\draw    (39,220) -- (111,220) -- (111,245) -- (39,245) -- cycle  ;
	\draw (42,224) node [anchor=north west][inner sep=0.75pt]   [align=left] {Electricity};
	% Text Node
	\draw    (293,65) -- (322,65) -- (322,90) -- (293,90) -- cycle  ;
	\draw (296,69) node [anchor=north west][inner sep=0.75pt]   [align=left] {CB};
	% Text Node
	\draw    (289,136) -- (329,136) -- (329,161) -- (289,161) -- cycle  ;
	\draw (292,140) node [anchor=north west][inner sep=0.75pt]   [align=left] {CHP};
	% Text Node
	\draw    (295,180) -- (324,180) -- (324,205) -- (295,205) -- cycle  ;
	\draw (298,184) node [anchor=north west][inner sep=0.75pt]   [align=left] {HP};
	% Text Node
	\draw    (463,99) -- (503,99) -- (503,124) -- (463,124) -- cycle  ;
	\draw (466,103) node [anchor=north west][inner sep=0.75pt]   [align=left] {Heat};
	% Text Node
	\draw    (450,220) -- (522,220) -- (522,243) -- (450,243) -- cycle  ;
	\draw (453,224) node [anchor=north west][inner sep=0.75pt]   [align=center] {Electricity};
	
	
\end{tikzpicture}

